Analysing Time-Stamped Co-Editing Networks in Software Development Teams using git2net

Data from software repositories have become an important foundation for the empirical study of software engineering processes. A recurring theme in the repository mining literature is the inference of developer networks capturing e.g. collaboration, coordination, or communication from the commit history of projects. Most of the studied networks are based on the co-authorship of software artefacts. Because this neglects detailed information on code changes and code ownership we introduce git2net, a scalable python software that facilitates the extraction of fine-grained co-editing networks in large git repositories. It uses text mining techniques to analyse the detailed history of textual modifications within files. We apply our tool in two case studies using GitHub repositories of multiple Open Source as well as a commercial software project. Specifically, we use data on more than 1.2 million commits and more than 25'000 developers to test a hypothesis on the relation between developer productivity and co-editing patterns in software teams. We argue that git2net opens up a massive new source of high-resolution data on human collaboration patterns that can be used to advance theory in empirical software engineering, computational social science, and organisational studies.

==> tools_entity_relationship_diagrams.tex <==
\newcommand{\ReplaceStr}[1]{%
	\IfSubStr{#1}{ }{%
		\StrSubstitute{#1}{ }{\_}}{#1}}

\makeatletter
    \pgfarrowsdeclare{crow's foot}{crow's foot}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0pt}{-5\pgfutil@tempdima}}%
        \pgfpathlineto{\pgfqpoint{-10\pgfutil@tempdima}{0pt}}%
        \pgfpathlineto{\pgfqpoint{0pt}{5\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-6pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-6pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-6pt}{4pt}}%
        \pgfusepathqstroke%
    }

    \pgfarrowsdeclare{omany}{omany}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0pt}{-5\pgfutil@tempdima}}%
        \pgfpathlineto{\pgfqpoint{-10\pgfutil@tempdima}{0pt}}%
        \pgfpathlineto{\pgfqpoint{0pt}{5\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}%
        \pgfpathcircle{\pgfpoint{-9pt}{0}}{3pt}%\pgfusepath{fill=white}
        \pgfusepathqstroke%
    }

    \pgfarrowsdeclare{one}{one}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-3pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-3pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-3pt}{4pt}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-5pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-5pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-5pt}{4pt}}%
        \pgfusepathqstroke%
    }
    \pgfarrowsdeclare{oone}{oone}
    {
        \pgfarrowsleftextend{+-.5\pgflinewidth}%
        \pgfarrowsrightextend{+.5\pgflinewidth}%
    }
    {
        \pgfutil@tempdima=0.6pt%
        %\advance\pgfutil@tempdima by.25\pgflinewidth%
        \pgfsetdash{}{+0pt}%
        \pgfsetmiterjoin%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-4pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-4pt}{-4pt}}%
        \pgfpathlineto{\pgfqpoint{-4pt}{4pt}}%
        \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
        \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}%
        \pgfpathcircle{\pgfpoint{-9pt}{0}} {3pt}
        \pgfusepathqstroke%
    }
    \makeatother

    \tikzset{
        entity/.code={
            \tikzset{
                % label=above:#1,
                name=#1,
                inner ysep=1mm,
                inner xsep=0mm,
                every entity/.try,
                fill=white,
                rounded corners,
                very thick,
                % rectangle split,
                % rectangle split parts=2,
                % general shadow={
                %     shadow xshift=0.0625in,
                %     shadow yshift=-0.0625in,
                %     opacity=0.5,
                %     fill=black!50
                % }
            }%
            \newcommand\entityname{#1}%
        },
        entity anchor/.style={matrix anchor=#1.center},
        every entity/.style={
                draw,
        },
        every property/.style={
            inner xsep=.1cm, inner ysep=0.05cm, anchor=west, text width=3.3cm
        },
        zig zag to/.style={
            rounded corners,
            to path={(\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget) \tikztonodes}
        },
        zig zag to/.default=0.5,
        one to one/.style={
            one-one, zig zag to, thick
        },
        one to oone/.style={
            one-oone, zig zag to, thick
        },
        one to many/.style={
            one-crow's foot, zig zag to, thick
        },
        one to omany/.style={
            one-omany, zig zag to, thick
        },
        oone to one/.style={
            oone-one, zig zag to, thick
        },
        oone to oone/.style={
            oone-oone, zig zag to, thick
        },
        oone to many/.style={
            -crow's foot, dashed, zig zag to, thick
        },
        oone to omany/.style={
            -omany, dashed, zig zag to, thick
        },
        many to one/.style={
            crow's foot-one, zig zag to, thick
        },
        many to oone/.style={
            crow's foot-, dashed, zig zag to, thick
        },
        many to many/.style={
            crow's foot-crow's foot, zig zag to, thick
        },
        many to omany/.style={
            crow's foot-omany, zig zag to, thick
        },
        omany to one/.style={
            omany-one, zig zag to, thick
        },
        omany to oone/.style={
            omany-, dashed, zig zag to, thick
        },
        omany to many/.style={
            omany-crow's foot, zig zag to, thick
        },
        omany to omany/.style={
            omany-omany, zig zag to, thick
        },
    }

    \newcommand{\prop}[1]{\node[name=\entityname-#1, every property/.try]{#1};}
    \newcommand{\properties}{\begingroup\catcode`\_=11\relax\processproperties}
    \newcommand{\processproperties}[1]{\endgroup%
        \newcommand\propertycode{}%
        \foreach \p in {#1}{%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\propertycode%
                \expandafter\expandafter\expandafter{\expandafter\propertycode\expandafter\prop\expandafter{\p}\\}%
        }%
        \propertycode%
    }

    \newcommand{\ERstr}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{str}}}};\\
    }
    \newcommand{\ERint}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{int}}}};\\
    }
    \newcommand{\ERfloat}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{float}}}};\\
    }
%    \newcommand{\ERlist}[2]{
%        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
%        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
%        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{list}}}};\\
%    }
    \newcommand{\ERdate}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{date}}}};\\
    }
    \newcommand{\ERbool}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{bool}}}};\\
    }
    \newcommand{\ERkey}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textit{KEY}}}};\\
    }
    \newcommand{\ERTODO}[2]{
        \node[name=\entityname-#1, every property/.try]{\scalebox{.75}[.75]{#2#1}};
        \node[name=\entityname-#1, every property/.try, red, text width=3.3cm, 
        align=right]{\textcolor{black!50}{\scalebox{.75}[.75]{\textbf{TODO}}}};\\
    }

    \newcommand{\entitynamenode}{%
    \node[every entity name/.try] (\entityname-name) {\MakeUppercase{\textbf{\entityname}}};
    \draw[thick, shorten <= 1mm, shorten >= 1mm] (\entityname-name.south west) -- (\entityname-name.south east);
    \\[1ex]
    }
    \tikzset{
      every entity name/.style={every property/.try, align=center, text 
      width=3.3cm}
    }
